Conformal Prediction for Distribution-to-Distribution Regression

Conformal Prediction (CP) provides a model-agnostic framework for constructing finite-sample prediction sets with coverage guarantees and has become a tool for reliable decision-making in high-risk settings. Recent advances have extended Split Conformal Prediction to increasingly complex learning problems, including multilabel, high-dimensional, and functional outputs. In this work, we study CP for Distribution-to-Distribution Regression, a setting of growing interest across many application domains. We show that a naive application of Split CP yields prediction sets that, while marginally valid, are non-interpretable, e.g., lacking a well-defined volume or a tractable sampling procedure, and of limited practical value. To overcome this, we propose a new conformal framework that operates in an orthogonal basis space, producing interpretable prediction sets while preserving coverage guarantees. We further develop an adaptive variant with asymptotic conditional coverage under mild assumptions. Empirical results on synthetic and real-world datasets validate the effectiveness of the proposed approach. The code is publicly available at https://github.com/tuanhacs/conformal_d2d.

==> Algorithms/LOO_estimation.tex <==
\begin{algorithm}[t]
\caption{LOO Estimator for $\mathbb{E}[\alpha_\delta(X_0)]$}
\label{alg: loo}
\begin{algorithmic}[1]

\Require Calibration subset $\mathcal C_a = \{(X_1^a,Y_1^a),\dots,(X_n^a,Y_n^a)\}$, Size budget function $\mathcal S(\cdot)$, slack $\delta \in (0,\zeta]$, truncation parameter $\varepsilon \in (0,1/2)$, Nonconformity score $s$.

\For{$k=1,\dots,n$}
    \State Define leave-one-out set:
    \begin{align*}
    \mathcal C_a^k \gets \mathcal C_a \setminus \{(X_k^a,Y_k^a)\}
    \end{align*}

    \State Compute scores:
    \begin{align*}
    s_i^{a,k} \gets s(\hat f(X_i^a),Y_i^a), \quad i \neq k
    \end{align*}

    \State Compute empirical quantile $\hat q_a^k(\alpha)$ from $\{s_i^{a,k}\}_{i \neq k}$

    \State Compute pseudo-level:
    \begin{align*}
    \alpha_\delta^k(X_k^a)
    \gets
    \inf\Big\{
    \alpha \in [\varepsilon,1-\varepsilon]:
    |\{y \in \mathcal Y : s(\hat f(X_k^a),y) \le \hat q_a^k(\alpha)\}|
    \le \mathcal S(X_k^a) - \delta
    \Big\}
    \end{align*}
\EndFor

\State Output estimator:
\begin{align*}
\hat \alpha_\delta
\gets
\frac{1}{n}\sum_{k=1}^n \alpha_\delta^k(X_k^a)
\end{align*}

\end{algorithmic}
\end{algorithm}

==> Algorithms/Main_method.tex <==
\begin{algorithm}[t]
\caption{Our proposed method for sCP under Truncated Prediction Set Size setting}
\label{alg: tpss_scp}
\begin{algorithmic}[1]
\Require Training set $\mathcal D_{\mathrm{train}}$, Calibration set $\mathcal C$, Test input $X_0$, Size budget function $\mathcal S(\cdot)$, slack $\delta \in (0,\zeta]$, truncation parameter $\varepsilon \in (0,1/2)$, Nonconformity score $s:\mathcal Y \times \mathcal Y \to \mathbb R$

\State Split $\mathcal C$ into two disjoint subsets of equal size:
\begin{align*}
\mathcal C_a=\{(X_1^a,Y_1^a),\dots,(X_n^a,Y_n^a)\},
\qquad
\mathcal C_c=\{(X_1^c,Y_1^c),\dots,(X_n^c,Y_n^c)\}.
\end{align*}

\State Train the prediction model $\hat f$ on the training data.

\For{$i=1,\dots,n$}
    \State Compute
    \begin{align*}
    s_i^{(a)} \gets s\big(\hat f(X_i^a),Y_i^a\big),
    \qquad
    s_i^{(c)} \gets s\big(\hat f(X_i^c),Y_i^c\big).
    \end{align*}
\EndFor

\State Define $\hat q_a(\alpha)\leftarrow$  the empirical $(1-\alpha)$-quantiles of $\{s_i^{(a)}\}_{i=1}^n$.
\State Define $\hat q_c(\alpha)\leftarrow$ the empirical $(1-\alpha)$-quantiles of $\{s_i^{(c)}\}_{i=1}^n$.

\State Compute the data-dependent level
\begin{align*}
\alpha_\delta(X_0)
\gets
\inf\Big\{
\alpha \in [\varepsilon,1-\varepsilon]
:
\big|
\{y \in \mathcal Y : s(\hat f(X_0),y)\le \hat q_a(\alpha)\}
\big|
\le \mathcal S(X_0)-\delta
\Big\}.
\end{align*}

\State Output the prediction set
\begin{align*}
C_\delta(X_0)
\gets
\{y \in \mathcal Y : s(\hat f(X_0),y)\le \hat q_c(\alpha_\delta(X_0))\}.
\end{align*}

\end{algorithmic}
\end{algorithm}
